Automatic Discovery of Novel Intents & Domains from Text Utterances

One of the primary tasks in Natural Language Understanding (NLU) is to recognize the intents as well as domains of users' spoken and written language utterances. Most existing research formulates this as a supervised classification problem with a closed-world assumption, i.e. the domains or intents to be identified are pre-defined or known beforehand. Real-world applications however increasingly encounter dynamic, rapidly evolving environments with newly emerging intents and domains, about which no information is known during model training. We propose a novel framework, ADVIN, to automatically discover novel domains and intents from large volumes of unlabeled data. We first employ an open classification model to identify all utterances potentially consisting of a novel intent. Next, we build a knowledge transfer component with a pairwise margin loss function. It learns discriminative deep features to group together utterances and discover multiple latent intent categories within them in an unsupervised manner. We finally hierarchically link mutually related intents into domains, forming an intent-domain taxonomy. ADVIN significantly outperforms baselines on three benchmark datasets, and real user utterances from a commercial voice-powered agent.

==> arXiv Discovering and Linking Novel User Intents from Text Utterances/conclusion.tex <==
\section{Conclusion}

We propose a novel and flexible multi-stage framework, \mname{}, to discover newly emerging, unknown intents and domains in large volumes of unlabeled text data. We first identify all input utterances likely to contain a novel intent. We next develop a network that learns discriminative deep features by maximizing inter-intent variance and minimize intra-intent variance between utterance pairs. We then transfer knowledge learned from intents seen during training to the unlabeled data containing novel intents. Finally, we hierarchically link mutually related intents into domains, to obtain a taxonomy of newly discovered intents and domains. We extensively evaluate \mname{} on three public benchmark datasets and real user utterances from a commercial dialog agent, and achieve state-of-the-art results across various empirical configurations. In future, we plan to (i) extend our proposed framework to handle input utterances consisting of multiple intents and/or domains per utterance; and (ii) use additional knowledge to better model human-perceived latent intents and domains.


==> arXiv Discovering and Linking Novel User Intents from Text Utterances/experiments.tex <==
\section{Evaluation}
\label{sec:evalution}

\subsection{Datasets and Experimental Setup}

%We use the following real-world datasets to test our proposed approach \mname{}, of discovering novel intents from unlabeled data and linking together mutually related intents: (i) SNIPS NLU benchmark~\cite{coucke2018} created by the company \textit{snips.ai}, (ii) ATIS NLU benchmark~\cite{dahl1994} from the flight reservation domain, (iii) Facebook semantic parsing dataset~\cite{gupta2018semantic}, and (iv) Internal NLU data\footnotemark from a commercial voice assistant. Statistics of these datasets are shown in Table~\ref{tab:stats}. 
We test \mname{} on the real-world datasets 
of SNIPS~\cite{coucke2018}%created by the company \textit{snips.ai}
, ATIS~\cite{dahl1994}%from the flight reservation domain
, Facebook's task-oriented semantic parsing (FTOP) data~\cite{gupta2018semantic}, and 
Internal NLU Data\footnotemark from a commercial voice assistant. 
For evaluation on SNIPS, ATIS and the Internal data, we completely remove all utterances associated with certain random sets of intents and domains from the training and validation sets, detailed in Table~\ref{tab:removed}. The FTOP dataset has intent types labeled as `unsupported', so we simply remove all utterances belonging to these intents while training \mname{}. Treating these removed intent and domain categories as novel (unseen), we then assess the efficacy of \mname{} in discovering these intents and domains during the testing phase. 
ATIS dataset intents are about airline reservations and are relatively similar to each other, while the SNIPS dataset consists of relatively dissimilar intent types. 
Our empirical configurations therefore holistically exhibit the performance of \mname{} when the novel intents being discovered have varying degrees of similarity with each other (or with the existing `seen' intents). 


\smallskip

\noindent \textbf{Hyperparameters:} %We now outline the exact implementation details and various hyperparameter values used in our algorithms. 
We used the English uncased BERT-Base model~\cite{devlin2018bert} in all steps of \mname{}. It has $12$ transformer layers, $768$ hidden states, and $12$ self-attention heads. We kept the dropout probability at $0.1$ and used the Adam optimizer~\cite{kingma2014adam} with parameters $\beta_1= 0.9$ and $\beta_2= 0.999$. We used slanted triangular learning rates~\cite{howard2018universal} for BERT with the base learning rate at $2e^{-5}$, and warm-up proportion at $0.1$. We empirically set the batch size to $64$, and the number of training epochs to $8$ for detecting instances with novel intents, and $15$ for discovering the latent intent categories. %, and save the best model on the validation set for testing.
To learn pairwise distances between utterances for clustering, we set $\alpha$ = $\beta$ = 1, and $m_1$ = $m_2$ = $m_3$ = 0.05. While discovering novel intent categories (Section~\ref{sec:stage2}), we used cosine similarity as the function `\textit{d(.)}' while computing $d(E(\bm{x}), E(\bm{x^p}))$, and euclidean distance as the function `\textit{f(.)}' while computing $f(Emb(\bm{x}), Emb(\bm{x^p}))$.
%Instead of saying 0, 0.5, 1: say i, j, k. Say in hyperparameters that we found 0,0.5,1 to work best for most datasets.
%m1=, m2=, m3=

\begin{comment}
The intents that we remove while training and aim to discover during evaluation for different datasets are:
\begin{enumerate}
\item SNIPS: Set 1: \textit{Weather, Restaurant}; and Set 2: \textit{AddToPlaylist, RateBook}.
\item ATIS: Set 1: \textit{airline, meal, airfare, day-name, distance}; and Set 2: \textit{ flight-time, flight-no, flight, ground-service, aircraft}. 
\item FTOP: Set 1:  \textit{unsupported, unsupported-event, unsupported-navigation, unintelligible}.
\item Internal NLU Dataset: we remove all intents present in the following domains: Set 1: \textit{Weather, Calendar, Todos}; Set 2: \textit{Sports, Local Search, Video, General Media, BookingsAndReservations}; Set 3: \textit{Recipe, Music, Shopping, Communication}; and Set 4: \textit{Global, Knowledge}.
\end{enumerate}
\end{comment}

\begin{table}[t]
\caption{Evaluating \mname{} on discovering novel intents and domains removed during training}
%\vspace{-0.6em}
\label{tab:removed} \centering
\small
\hskip-0.4cm\begin{tabularx}{1.03\linewidth}{L{0.15}|L{1.4}|L{0.17}|L{0.13}|L{0.15}}
\hline
\textbf{Dataset} & \textbf{Sets of intents removed from training data for evaluation} & \textbf{\# of data samples} & \textbf{Vocab size} & \textbf{Avg. text len.}  \\
\hline
SNIPS & \textbf{Set 1}: \textit{Weather, Restaurant}; \textbf{Set 2}: \textit{AddToPlaylist, RateBook} & 13.8K & 10.9K & 9.05 \\
ATIS & \textbf{Set 1}: \textit{airline, meal, airfare, day-name, distance}; \textbf{Set 2}: \textit{ flight-time, flight-no, flight, aircraft, ground-service}  & 5.87K & 0.87K & 11.2  \\
FTOP & \textbf{Set 1}:  \textit{unsupported, unsupported-event, unsupported-navigation, unintelligible} & 44.78K & 16.69K  & 8.93  \\
Internal NLU Dataset & \textbf{Set 1}: \textit{Weather, Calendar, Todos}; \textbf{Set 2}: \textit{Bookings\&Reservations, Sports, Local Search, Video, General Media}; \textbf{Set 3}: \textit{Recipe, Music, Shopping, Communication}; \textbf{Set 4}: \textit{Global, Knowledge}  & 3.16M & 26.7K & 3.72 \\
\hline
\end{tabularx}
\end{table}


%domain information is not available for SNIPS/ATIS, we only use x, xi and x, xk.

\begin{comment}
\begin{table}[t]
\caption{Statistics of the datasets used in our experiments}
%\vspace{-0.6em}
\label{tab:stats} \centering
\small
\begin{tabularx}{\linewidth}{L{0.87}|L{0.23}|L{0.19}|L{0.35}|L{0.36}}
\hline
\textbf{Dataset} & \textbf{SNIPS} & \textbf{ATIS} & \textbf{FTOP} & \textbf{Internal Dataset} \\
\hline
\# of data samples & 13.8K & 5.87K & 44.78K & 3.16M \\
Vocabulary size & 10.9K & 0.87K & 16.69K & 26.7K \\
Avg. utterance length & 9.05 & 11.2 & 8.93 & 3.72 \\
\hline
\end{tabularx}
\end{table}
\end{comment}

\footnotetext{Customer utterances from a voice-powered virtual assistant, whose name we omit for the double-blind review purpose.}


\subsection{Baselines and Evaluation Metrics} 

%We compare the first step of our proposed approach of detecting utterances with novel intents \textbf{``\mname{} \textit{(multi unseen + DOC)}"} with the following baseline approaches in Table~\ref{tab:stage1}: 
%(i) \textbf{DOC}~\cite{shu2017doc}: an open-world classification approach with a 1-vs-rest sigmoid layer on top of a CNN. It tightens the sigmoid decision boundary by learning statistical class-specific confidence thresholds. (ii) \textbf{IntentCapsNet}~\cite{xia2018}: a zero-shot learning method that uses capsule neural networks to discover emerging intents. (iii) \textbf{LOF-LMCL}~\cite{lin2019deep}: it uses a local outlier detection method on top of a Bi-LSTM trained with a large margin cosine loss to distinguish between intents seen and unseen during training. (iv) \textbf{\mname{} \textit{(one unseen)}/\mname{} \textit{(one unseen + DOC)}}: variants of \mname{} that use a single unseen class while training our classification model, with and without the additional check employing the class-specific confidence thresholds per the DOC heuristic. (v) \textbf{\mname{} \textit{(multi unseen)}}: \mname{} with multiple unseen classes while training our classification model and without the DOC heuristic. 
%For evaluation, we use the standard classification metrics of accuracy and F1-score.


We designate the first step of our proposed approach of detecting utterances with novel intents as \textbf{``\mname{} \textit{(m-unseen + DOC)}"}, and compare it with the following state-of-the-art approaches in Table~\ref{tab:stage1}: 

\smallskip
\noindent \noindent (i) \textbf{DOC}~\cite{shu2017doc}: uses a CNN with a 1-vs-rest sigmoid layer on top. It tightens the sigmoid decision boundary by learning class-specific confidence thresholds to detect novel intents. 

\noindent (ii) \textbf{IntentCapsNet}~\cite{xia2018}: uses capsule neural networks in a zero shot setting to discover newly emerging intents. 

\noindent (iii) \textbf{LOF-LMCL}~\cite{lin2019deep}: uses local outlier detection on top of a Bi-LSTM trained with a large margin cosine loss to classify seen and unseen intents.% seen and unseen during training. 

\noindent (iv) \textbf{\mname{} \textit{(1-unseen)}/\mname{} \textit{(1-unseen + DOC)}}: variants of \mname{} using an \textit{(S+1)}-class classification model (Section~\ref{sec:stage1}), with and without the additional check %employing the class-specific confidence thresholds 
per the DOC heuristic. 

\noindent (v) \textbf{\mname{} \textit{(m-unseen)}}: \mname{}'s \textit{(S+1)}-th class split into $m$ novel classes, without the DOC heuristic. 

\smallskip

\begin{table*}[t]
\centering
\caption{F1-score of various approaches for detecting if an utterance contains a novel intent or not.} %Different Sets denoting different intents removed from the training set and appearing as novel intents in the test set.}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabularx}{\linewidth}{L{0.87}|L{0.11}|L{0.11}|L{0.11}|L{0.11}|L{0.25}|L{0.11}|L{0.11}|L{0.11}|L{0.11}} \hline
  \textbf{Approach} & \multicolumn{2}{c|}{\textbf{SNIPS}} & \multicolumn{2}{c|}{\textbf{ATIS}} & \textbf{FTOP} & \multicolumn{4}{|c}{\textbf{Internal Dataset}}  \\\cline{2-10}
    &  \textbf{Set1}   & \textbf{Set2}  &  \textbf{Set1}  & \textbf{Set2}  &  \textbf{Set1}  &  \textbf{Set1}  & \textbf{Set2} & \textbf{Set3}  & \textbf{Set4}  \\%\cline{2-13}
    %&  FT:0.83  & S$\leftarrow$T  &  S$\rightarrow$T  & S$\leftarrow$T  &  S$\rightarrow$T  & S$\leftarrow$T &  S$\rightarrow$T  & S$\leftarrow$T &  S$\rightarrow$T  & S$\leftarrow$T &  S$\rightarrow$T  & S$\leftarrow$T \\ \hline
    \hline
  DOC~\cite{shu2017doc}  & 0.73 & 0.69 & 0.71 & 0.7 & 0.76 & 0.7 & 0.73 & 0.72 & 0.71 \\ 
  IntentCapsNet~\cite{xia2018} & 0.81 & 0.77 & 0.7 & 0.75 & 0.8 & 0.82 & 0.83 & 0.78 & 0.8 \\ 
  LOF-LMCL~\cite{lin2019deep} & 0.79 & 0.73 & 0.68 & 0.74 & 0.78 & 0.84 & 0.8 & 0.82 & 0.81\\ 
  \mname{} \textit{(1-unseen)} & 0.76 & 0.73 & 0.68 & 0.72 & 0.78 & 0.77 & 0.75 & 0.79 & 0.8 \\ 
  \mname{} \textit{(1-unseen+DOC)} & 0.85 & 0.81 & 0.73 & 0.8 & 0.87 & 0.86 & 0.87 & 0.88 & 0.86\\ 
  \mname{} \textit{(m-unseen)} & 0.78 & 0.75 & 0.7 & 0.75 & 0.8 & 0.8 & 0.8 & 0.82 & 0.84 \\ 
  \mname{} \textit{(m-unseen+DOC)} & \textbf{0.9} & \textbf{0.87} & \textbf{0.78} & \textbf{0.84} & \textbf{0.9} & \textbf{0.9} & \textbf{0.92} & \textbf{0.9} & \textbf{0.9} \\ 
\hline
\end{tabularx}
%}
\label{tab:stage1}
\end{table*}


\begin{table*}[t]
\centering
\caption{Discovering the latent intent types for utterances with novel intents. `\#int.' shows the number of discovered intents, `GT' denotes the true number of intents, and `Pur.' denotes cluster purity.}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabularx}{1.02\linewidth}{L{0.66}|L{0.12}|L{0.11}|L{0.12}|L{0.09}|L{0.12}|L{0.11}|L{0.12}|L{0.09}|L{0.12}|L{0.11}|L{0.12}|L{0.08}} \hline
  \textbf{Approach} & \multicolumn{4}{c|}{\textbf{SNIPS Set 1 (GT = 2)}} & \multicolumn{4}{c|}{\textbf{SNIPS Set 2 (GT = 2)}} & \multicolumn{4}{|c}{\textbf{FTOP Set 1 (GT = 4)}}  \\\cline{2-13}
    &  \footnotesize{\bf \#int.} & \textbf{NMI}  &  \textbf{Pur.}   &  \textbf{F1} &  \footnotesize{\bf \#int.} & \textbf{NMI}  &  \textbf{Pur.} &  \textbf{F1} &  \footnotesize{\bf \#int.} & \textbf{NMI}  &  \textbf{Pur.}   &  \textbf{F1}
    \\%\cline{2-13}
    \hline
  \mname{} \textit{(clf+hier)} & \textbf{3} & 0.78 & 0.9 & 0.76 & \textbf{3} & 0.7 & 0.8 & 0.69 & 24 & 0.4 & 0.56 & 0.38\\ 
  \mname{} \textit{(triplet+hier)} & 4 & 0.71 & 0.81 & 0.69 & 5 & 0.65 & 0.76 & 0.66 & 48 & 0.36 & 0.51 & 0.35\\ 
  \mname{} \textit{(ProdLDA)} & NA & 0.71 & 0.84 & 0.72 & NA & 0.66 & 0.79 & 0.68 & NA & 0.42 & 0.53 & 0.38\\ 
  \mname{} \textit{(pair+RCC)} & \textbf{3} & 0.79 & 0.9 & 0.77 & \textbf{3} & 0.7 & 0.8 & 0.7 & 30 & \textbf{0.5} & \textbf{0.63} & 0.41\\ 
  \mname{} \textit{(pair+hier)} & \textbf{3} & \textbf{0.8} & \textbf{0.92} & \textbf{0.78} & \textbf{3} & \textbf{0.72} & \textbf{0.83} & \textbf{0.71} & \textbf{19} & 0.46 & 0.61 & \textbf{0.51}\\ 
\hline
\end{tabularx}
%}
\label{tab:stage21}
\end{table*}


\begin{table*}[t]
\centering
\caption{Discovering the actual, latent novel intents and novel domains of input utterances. For Internal Data Sets 1 and 2, the first two columns show the number of new intents (\#int.) and new domains (\#dom.) discovered respectively. `GT ($d$, $i$)' denotes the true number of domains $d$ and intents $i$.}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabularx}{\linewidth}{L{0.65}|L{0.15}|L{0.17}|L{0.11}|L{0.14}|L{0.1}|L{0.16}|L{0.17}|L{0.11}|L{0.14}|L{0.1}} \hline
  \textbf{Approach} & \multicolumn{5}{c|}{\textbf{Internal Data Set 1 (GT = 3, 22)}} & \multicolumn{5}{|c}{\textbf{Internal Data Set 2 (GT = 5, 53)}}  \\\cline{2-11}
    &  \footnotesize{\bf \# int.} & \footnotesize{\bf \# dom.} & \textbf{NMI}  &  \textbf{Purity}   &  \textbf{F1} &  \footnotesize{\bf \# int.} & \footnotesize{\bf \# dom.} & \textbf{NMI}  &  \textbf{Purity} &  \textbf{F1}
    \\%\cline{2-13}
    \hline
  \mname{} \textit{(clf+hier)} & 108 & 35 & 0.53 & 0.69 & 0.48 & 178 & 71 & 0.41 & 0.64 & 0.36  \\ 
  \mname{} \textit{(triplet+hier)} & 206 & 51 & 0.52 & 0.63 & 0.41 & 205 & 65 & 0.33 & 0.61 & 0.31  \\ 
  \mname{} \textit{(ProdLDA)} & NA & NA & 0.56 & 0.7 & 0.55 & NA & NA & 0.4 & 0.69 & 0.42   \\ 
  \mname{} \textit{(pair+RCC)} & 91 & 40 & 0.55 & 0.73 & 0.52 & 188  & 57 & 0.5 & 0.74 & 0.5 \\ 
  \mname{} \textit{(pair+hier)} & \textbf{74} & \textbf{29} & \textbf{0.6} & \textbf{0.75} & \textbf{0.6} & \textbf{167} & \textbf{36}  & \textbf{0.57} & \textbf{0.75} & \textbf{0.55} \\ 
\hline
\end{tabularx}
%}
\label{tab:stage22}
\end{table*}


%For evaluating the next two steps of discovering the actual intent categories in the user utterances and linking the newly discovered intents into domains, we denote our proposed method as \textbf{``\mname{} \textit{(pairwise emb)}"}, i.e. using distances between embeddings learned via our pairwise training technique as input to hierarchical clustering. We compare it with the following approaches: (i) \textbf{\mname{} \textit{(clf emb)}}: uses the representation learned by the 2nd to last BERT layer of our classification model in Figure~\ref{fig:stage1}, as input to hierarchical clustering. (ii) \textbf{\mname{} \textit{(triplet emb)}}: uses embeddings trained with a triplet loss function consisting of utterance triplets $(x, x^-, x^+)$, as input to hierarchical clustering. $x^-$ and $x^+$ refer to utterances containing the same domain and intent, and different domain and intent as utterance $x$ respectively. (iii) \textbf{\mname{} \textit{(ProdLDA)}}: uses a neural topic modeling algorithm ProdLDA~\cite{srivastava2017autoencoding} in order to discover the novel intent categories in place of clustering. Since ProdLDA requires the number of topics as input, we give it the number of clusters output by ``\mname{} \textit{(pairwise emb)}". We denote the most likely topic for each utterance as its intent. (iv) \textbf{\mname{} \textit{(pairwise + RCC)}}: uses embeddings learned via our pairwise margin loss function as input to the Robust Continuous Clustering algorithm (RCC)~\cite{shah2017robust}, instead of hierarchical clustering. 


The first stage of discovering utterances with novel intents (Section~\ref{sec:stage1}) is evaluated using the standard F1-score metric. For evaluating the next two stages of discovering the actual intent categories in the user utterances and linking the newly discovered intents into domains (Sections~\ref{sec:stage2} and~\ref{sec:stage3}), we designate our proposed method as \textbf{``\mname{} \textit{(pair+hier})"}, i.e. using distances between embeddings learned via our pairwise margin loss function as input to hierarchical clustering. %We compare it with these baselines:
As per our knowledge, work in the literature only detects if text utterances contain novel intents or not, and does not identify the actual, latent intent categories in unlabeled text. Therefore, we compare \mname{} with its own variant baselines: %different variants of ADVIN in Tables 4 and 5. %We also experimented with a number of different clustering approaches (apart from hierarchical clustering), but did not include these results due to lack of space.

\smallskip

\noindent (i) \textbf{\mname{} \textit{(clf+hier)}}: uses the representation learned by the 2nd to last BERT layer of our classification model in Figure~\ref{fig:stage1}, as input to hierarchical clustering. 

\noindent (ii) \textbf{\mname{} \textit{(triplet+hier)}}: uses embeddings learned by a triplet network~\cite{schroff2015facenet} as input to hierarchical clustering. The inputs to the network are utterance triplets $(x, x^-, x^+)$. $x^-$ and $x^+$ contain the same domain and intent, and different domain and intent as utterance $x$ respectively. 

\noindent (iii)  \textbf{\mname{} \textit{(ProdLDA)}}: uses a neural topic modeling method ProdLDA~\cite{srivastava2017autoencoding} to discover novel intent categories, instead of clustering. %We denote the most likely topic for each utterance as its intent. 
ProdLDA requires the number of topics as input, so we give it the number of clusters output by ``\mname{} \textit{(pair+hier)}".

\noindent (iv) \textbf{\mname{} \textit{(pair+RCC)}}: uses embeddings learned via our pairwise loss function as input to the Robust Continuous Clustering algorithm (RCC)~\cite{shah2017robust}, instead of hierarchical clustering. 
\smallskip

Ground truth intent and domain labels are available for the various experimental data Sets we used for evaluation (Table~\ref{tab:removed}). We thus use the following standard clustering metrics to evaluate the novel intents and domains discovered: (i) Comparing the number of discovered intents and domains to the ground truth number. (ii) Normalized Mutual Information (NMI): a normalization of the mutual information by a generalized mean of the entropy of the ground truth and the entropy of the predicted cluster labels. %, to scale the result between 0 (no mutual information) and 1 (perfect correlation). 
(iii) Purity: the extent to which a cluster contains utterances with a single intent or domain. (iv) F1 score.

\subsection{Results}

\noindent \textbf{Baseline Comparison: } Table~\ref{tab:stage1} shows the F1-score of various approaches, on classifying an intent as novel or not on different datasets with different dataset configurations. We observe that our approach using an $(S+m)$-class classifier during training and the DOC heuristic, ``\mname{} \textit{(m-unseen+DOC)}", outperforms all baselines on all datasets by at least 6\% F1 score points. \mname{} also outperforms the zero shot IntentCapsNet model (that uses relevant information available beforehand about the new test intents to be discovered), without using any prior knowledge about the novel intents or domains.


Tables~\ref{tab:stage21} and~\ref{tab:stage22} show the performance of different approaches in discovering intent categories for the utterances containing novel intents as predicted in Table~\ref{tab:stage1}. We observe that our proposed approach ``(\mname{} + \textit{pair+hier})" using distances learned via our pairwise loss training method along with hierarchical clustering outperforms the rest of the baselines. The learned intent-clusters have a purity value more than 80\% for the SNIPS dataset. Purity decreases to $61\%$ for FTOP, primarily because semantically diverse utterances have been given the same ground truth intent label of \textit{`unsupported'} or \textit{`unsupported-event'}. The `NA' value for ``\mname{} \textit{(ProdLDA)}" in the column `\# int.' denotes that the \textit{ProdLDA} algorithm by design does not output the number of new intents discovered. It takes this as input in the form of the number of topics. We observe similar empirical trends as above on ATIS Sets 1 and 2, and Internal NLU Data Sets 3 and 4. In the interests of space, we do not present these results.

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=8.7cm,height=6cm]{Figures/tsne} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
\caption{Visualizing embeddings learned by \mname{} for novel intents discovered within the \textit{`unsupported'} FTOP category.}
\label{fig:tsne}
\end{figure}
\end{comment}



Our technique discovers $1.5$-$4.5$ times more novel intents than present in the ground truth, as seen from the `\# int.' columns in Tables~\ref{tab:stage21} and~\ref{tab:stage22}. To investigate this further, we use t-SNE~\cite{maaten2008visualizing} to visualize the embeddings learned by training our proposed \mname{} method, for the utterances belonging to the \textit{`unsupported'} intent category of the FTOP dataset. In Figure~\ref{fig:tsne}, each color represents a different novel intent category discovered. We also show the most frequent utterance words present in each newly emergent intent. 
We observe that \textit{`Unsupported'} has been split up by \mname{} into $7$ finer-grained, semantically sensible novel intents. For instance, the utterances \textit{``What city has the most traffic in the US"} and \textit{``Family friendly bars near me"}, from the \textit{`unsupported'} intent category, have been separated by \mname{} into different intent categories.  Figure~\ref{fig:tsne} also explains the lower performance values in Table~\ref{tab:stage21} for the FTOP dataset. We thus find that \mname{} largely learns semantically appropriate, discriminative representations for the newly emerging intents (also echoed by our user study in Table~\ref{tab:user study}).


\begin{figure}
\begin{minipage}[c][7cm][t]{.5\textwidth}
  \vspace*{\fill}
  \centering
  {\label{fig:tsne}\includegraphics[width=8.6cm,height=6cm]{tsne}}
  \subcaption{}
\end{minipage}%
\begin{minipage}[c][7cm][t]{.5\textwidth}
  \vspace*{\fill}
  \centering
  {\label{fig:num_ood_intents}\includegraphics[width=6cm,height=2.8cm]{num_ood_intents_f1}}
  \subcaption{}
  \par\vfill
  {\label{fig:num_ood_intents}\includegraphics[width=6cm,height=2.8cm]{num_ood_intents_f1}}
  \subcaption{}
\end{minipage}
\caption{(a) Visualizing embeddings learned by \mname{} for novel intents discovered within the \textit{`unsupported'} FTOP category. The figure also shows the varying F1 score averaged across (b) number of OOD intent classes and (c) number of labeled OOD instances, given as training data for Stage I.}
\end{figure}


\begin{comment}
\begin{figure}
\centering
\sbox{\measurebox}{%
  \begin{minipage}[b]{.4\textwidth}
  \hspace{-1.5cm}
  \subfloat
    []
    {\label{fig:tsne}\includegraphics[width=8.6cm,height=6cm]{Figures/tsne}}
  \end{minipage}}
\usebox{\measurebox}
\qquad
\begin{minipage}[b][\ht\measurebox][s]{.4\textwidth}
\centering
\subfloat
  []
  {\label{fig:num_ood_intents}\includegraphics[width=6cm,height=2.8cm]{Figures/num_ood_intents_f1}}

\vfill

\subfloat
  []
  {\label{fig:num_ood_data}\includegraphics[width=6cm,height=2.8cm]{Figures/num_ood_data_f1}}
\end{minipage}

\caption{(a) Visualizing embeddings learned by \mname{} for novel intents discovered within the \textit{`unsupported'} FTOP category. The figure also shows the varying F1 score averaged across (b) number of OOD intent classes and (c) number of labeled OOD instances, given as training data for Stage I.}
\end{figure}
\end{comment}


\begin{comment}
\begin{table}[H]
    \hskip-0.5cm\begin{minipage}{.1\linewidth}
      \centering
      \caption{F1-scores evaluating \mname{}'s prediction on unseen utterance pairs containing the same novel intent or not, w.r.t user study annotations. Parentheses show F1-scores using the dataset-provided annotations as ground truth.}
    \label{tab:user study}
      \begin{tabular}{c|c|c} \hline
  \textbf{Approach} & \textbf{FTOP} & \textbf{Internal} \\ \hline
  \mname{} \textit{(clf+hier)} & 0.66 (0.6) & 0.6 (0.68) \\ 
  \mname{} \textit{(triplet+hier)} & 0.6 (0.57) & 0.55 (0.61)  \\ 
  \mname{} \textit{(ProdLDA)} & 0.65 (0.56) & 0.54 (0.61)  \\ 
  \mname{}\textit{(pair+RCC)} & 0.64 (0.6) & 0.56 (0.64)  \\ 
  \mname{} \textit{(pair+hier)} & 0.7 (0.61) & 0.61 (0.71)  \\ 
\hline
\end{tabular}
%}
    \end{minipage}
    \hskip0.5cm\begin{minipage}{1.3\linewidth}
      \centering
      \caption{Performance of \mname{} of discovering intent categories within unlabeled utterances containing novel intents, on providing limited supervision as pairwise constraints. Parentheses show the results without providing supervision.}
    \label{tab:supervision}
      \begin{tabular}{c|c|c|c|c} \hline
  \textbf{Dataset} & \textbf{\# int.} & \textbf{NMI} & \textbf{Purity} & \textbf{F1}
    \\%\cline{2-13}
    \hline
  SNIPS S1 & 2 (3) & 0.82(2\%) & 0.94(2\%) & 0.85(7\%) \\ 
  ATIS S1 & 12(13) & 0.74(2\%) & 0.77(4\%) & 0.75(3\%)  \\ 
  FTOP & 17(19) & 0.5(4\%) & 0.64(3\%) & 0.54(3\%)  \\ 
  Internal 1 & 45(56) & 0.65(5\%) & 0.75(4\%)  &  0.65(3\%) \\ 
  Internal 2 & 82(92) & 0.58(4\%) & 0.7(1\%)  & 0.61(3\%)  \\ 
  Internal 3 & 90(131) & 0.6(4\%) & 0.75(3\%)  & 0.6(3\%)  \\ 
  Internal 4 & 127(141) & 0.62(3\%) & 0.69(2\%)  &  0.61(2\%) \\ 
\hline
\end{tabular}
    \end{minipage}
  \end{table}
\end{comment}


%\begin{comment}
\begin{table}[t]
\centering
\caption{Evaluating \mname{}'s prediction of utterance pairs containing the same novel intent or not. Columns show F1 scores w.r.t  using (i) user study and (ii) dataset-provided annotations as ground truth.}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabularx}{1.03\linewidth}{L{0.45}|L{0.78}|L{0.77}} \hline
  \textbf{Approach} & \textbf{FTOP:F1 user study(F1 Dataset)} & \textbf{Internal:F1 user study(F1 Dataset)} \\ \hline
  \mname{} \textit{(clf+hier)} & 0.66 (0.6) & 0.6 (0.68) \\ 
  \mname{} \textit{(triplet+hier)} & 0.6 (0.57) & 0.55 (0.61)  \\ 
  \mname{} \textit{(ProdLDA)} & 0.65 (0.56) & 0.54 (0.61)  \\ 
  \mname{} \textit{(pair+RCC)} & 0.64 (0.6) & 0.56 (0.64)  \\ 
  \mname{} \textit{(pair+hier)} & 0.7 (0.61) & 0.61 (0.71)  \\ 
\hline
\end{tabularx}
%}
\label{tab:user study}
\end{table}


\begin{table}[t]
\centering
\caption{\mname{} discovering new intent categories for unlabeled utterances with novel intents, using limited supervision as pairwise constraints. Parentheses show original results without using supervision.}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabularx}{\linewidth}{L{0.445}|L{0.345}|L{0.41}|L{0.41}|L{0.39}} \hline
  \textbf{Dataset} & \textbf{\# intents} & \textbf{NMI} & \textbf{Purity} & \textbf{F1 score}
    \\%\cline{2-13}
    \hline
  SNIPS Set 1 & 2 (3) & 0.82 (0.8) & 0.94 (0.92) & 0.85 (0.78) \\ 
  ATIS Set 1 & 12 (13) & 0.74 (0.72) & 0.77 (0.73) & 0.75 (0.72)  \\ 
  FTOP Set 1 & 17 (19) & 0.5 (0.46) & 0.64 (0.61) & 0.54 (0.51)  \\ 
  Internal Data Set 1 & 45 (56) & 0.65 (0.61) & 0.75 (0.71)  &  0.65 (0.62) \\ 
  Internal Data Set 2 & 82 (92) & 0.58 (0.54) & 0.7 (0.69)  & 0.61 (0.58)  \\ 
  %Internal Data Set 3 & 90 (131) & 0.6 (0.56) & 0.75 (0.72)  & 0.6 (0.57)  \\ 
  %Internal Data Set 4 & 127 (141) & 0.62 (0.59) & 0.69 (0.67)  &  0.61 (0.59) \\ 
\hline
\end{tabularx}
%}
\label{tab:supervision}
\end{table}

%\end{comment}

\smallskip

\noindent \textbf{Effect of OOD training data: }
We analyze the effect of the labeled OOD instances given as training input to Stage I (detecting utterances with novel intents) of \mname{}. Figures~\ref{fig:num_ood_intents} and~\ref{fig:num_ood_data} show that the performances of both Stage I (Section~\ref{sec:stage1}) and II (Section~\ref{sec:stage2}) of \mname{} improve with increase in the number of (i) OOD intent classes, and (ii) OOD training data examples; up to a particular threshold `m' for the Internal NLU Data Set I. Increasing `m' beyond this value leads to a performance drop. We also observe that the presence of finer-grained labeled utterances (e.g. the intent labels of ATIS) in the OOD data has a higher performance impact, than the coarser-grained intent labels (e.g. FTOP intents). 
We find similar trends for the other datasets also, but do not present them due to space constraints. 

\smallskip

\noindent \textbf{Linking Intents to form Domains: }
There is no domain information available for the SNIPS, ATIS and FTOP data. Hence, we only evaluate the performance of linking intents into domains on the Internal dataset. The column of `\# dom.' in Table~\ref{tab:stage22} for Internal Data Sets 1 and 2 shows the number of newly discovered domains by \mname{} after linking mutually related newly discovered intents. 
As earlier, \mname{} obtains a finer-grained grouping of novel intents into novel domains. It finds $2$-$3$ times more number of domains than the dataset annotations. On further inspection, we found that the domains for the Internal datasets have been created by collating intents satisfying common business goals or customer needs, and are less geared towards semantics. Contrarily, \mname{} focuses on the semantic meaning of the utterances and performs a more fine-grained categorization of newly emerging intents into domains. This leads to a slight discord between the domains uncovered by \mname{}, and the domain annotations in the dataset. Such an over estimation of the number of novel intents or domains 
is often acceptable in a practical setting, since the granularity of domains and intents learned by \mname{} can be easily `coarsened' by merging together certain novel intents or domains, 
%should contain the same novel intent or domain can be grouped together 
based on downstream requirements. One way to do this is by soliciting human feedback %based on downstream application requirements 
(see Table~\ref{tab:supervision}). 

\smallskip

\noindent \textbf{User Study: }
To compare the intent and/or domain labels provided with the datasets and human perception of novel intents and domains while evaluating \mname{}, we conduct a \textit{user study} on the FTOP and Internal datasets.  We recruit crowd workers on Amazon Mechanical Turk for the FTOP data and employees familiar with the Internal Dataset for this purpose. We provide a set of random utterance pairs predicted as having novel intents to the annotators, and ask them to indicate whether the pair is likely to belong to the same intent category or not. 
For both datasets we compute the F1-score in Table~\ref{tab:user study}, by comparing the output of \mname{} with that of the human annotators, for $2500$ FTOP utterance pairs (inter-annotator agreement Cohen's $\kappa = 0.78$) and $1100$ Internal dataset utterance pairs (Cohen's $\kappa = 0.9$). 
We observe that `\mname{} (\textit{pair+hier})' trained with the pairwise margin loss and hierarchical clustering significantly outperforms all baselines by at least 5\% on both datasets with respect to human evaluation.   

\smallskip

\noindent \textbf{Introducing Limited Supervision: }
There is often some partial supervision or background knowledge already known to humans or provided by domain experts, regarding the unlabeled user utterances. Utilizing this can enhance the quality of the novel intents and domains discovered by \mname{}. Therefore, we test \mname{} in a semi-supervised setting, instead of the unsupervised hierarchical clustering, where we provide limited prior knowledge in the form of two types of pairwise constraints: (i) \textit{must-link}, for the utterances that must belong to the same novel intent category, and (ii) \textit{cannot-link}, for the utterances that cannot contain the same novel intent. We incorporate the constraints during hierarchical clustering by modifying the learned distance values between the utterance pairs. We show in Table~\ref{tab:supervision} the performance of \mname{}, while randomly selecting $3$ groups of $4$ utterances each for the \textit{must-link} and \textit{cannot-link} constraints. Thus, supervision is provided for $<25$ utterances. We observe a 2-8\% gain %in the number of discovered intents, NMI, cluster purity and F1 metrics across various datasets. 
across various metrics and datasets. 
This experiment demonstrates that \mname{} can be easily extended to a semi-supervised setting, and minimal supervision if available, can significantly improve the quality of the discovered intents and domains over an unsupervised setting. 


==> arXiv Discovering and Linking Novel User Intents from Text Utterances/introduction.tex <==
\section{Introduction}

Numerous everyday gadgets like mobile phones or smart speaker devices consist of an NLU component to automatically understand the semantics %, particularly the intentions
of user requests. %The action to be taken by the system is then decided based on the intent identified. 
Comprehending the \textit{intent} and/or \textit{domain} (groups of mutually related intents) of users' natural language utterances is a key task in these devices. Deep learning models have been proposed in the literature for intent detection in diversely expressed utterances, to avoid additional feature engineering~\cite{bhargava2013,kim2016intent,liu2016attention,sun2016weakly,zhang2016joint,kim2017onenet,goo2018slot}. %, and identify relevant entities linked with those intents (slot filling). 
But most models are supervised or semi-supervised, i.e. they require sufficient labeled data, and can only handle a fixed number of intents and domains \textit{seen} during model training.
%This inhibits the range of functionalities that the users of these voice assistants can enjoy.
However, user interactions with voice-powered agents generate large amounts of unlabeled conversational text. This data often contains newly emergent, \textit{unseen} domains and intents not encountered by the learning models before. %, and is expensive to label.
Expanding the capabilities of voice assistants to account for these new intents and domains would require expensive and time-consuming human labeling efforts each time a new skill, functionality or intent is to be added. Thus, it is crucial to be able to learn effectively from unlabeled text.

Zero shot techniques~\cite{kumar2017zero,xia2018} recognize intents for which no labeled training data is available. However, they require the number of the new intent types, and some prior knowledge about the new intents to be discovered to be available at test time. Such information may be unfeasible to obtain. 
Efforts have been made to break the closed-world assumption in computer vision~\cite{scheirer2014probability,bendale2015towards,bendale2016towards,fei2016breaking} as well as in the NLU literature~\cite{shu2017doc,kim2018joint,vedula2019towards,lin2019deep}. This is the paradigm of \textit{open world learning} or \textit{open set recognition}, that identifies instances with labels unseen during training. 
%These works classify instances from the \textit{seen} (during training) classes and reject instances that do not belong to any seen class as an \textit{unseen} (during training) or novel class. 
However, the task of discovering the actual latent categories in the instances identified as containing unseen labels is relatively under explored. \cite{shu2018unseen} attempted this for image classification, but their model could not always outperform baselines. \cite{vedula2019towards} developed a sequence tagging approach to discover unseen intents in dialog. However, unlike our proposed framework, their method (i) is restricted to intents containing an action or activity to be performed; (ii) is customized for longer utterances containing additional background context such as customer support conversations; and (iii) does not recognize an intent expressed in different ways semantically as the same intent, or group related novel intents into novel domains. 
In this work, we attempt to bridge the gap between detecting utterances belonging to new intents/domains and actually discovering a taxonomy of those new intents/domains. Though we address the problem of novel user intent and domain discovery, our technique can easily be applied to any open classification setting. 

We propose a novel three-stage framework called \mbox{\textit{\mname{}}} (\underline{A}utomatic \underline{D}iscovery of no\underline{V}el \underline{I}ntents and Domai\underline{N}s). It automatically discovers user intents and domains in massive, unlabeled text corpora, \textit{without} any prior knowledge about the intents or domains that the text may comprise of. 
Similar to an open classification setting, our method first leverages a multi-layer transformer network, BERT~\cite{devlin2018bert}, to determine if the text input is likely to contain a novel, unseen intent or not. In the next step, \mname{} discovers the latent intent categories in the above identified input utterances in an unsupervised manner, via a knowledge transfer component. %We do this by transferring the knowledge learnt from an utterance corpus labeled with intents seen during training.  
Finally, \mname{} hierarchically links semantically related groups of the newly discovered intents to form new domains. 
\mname{} is a generic algorithm and we empirically demonstrate that it is equally effective across several task domains and fields. %The gains obtained can further be improved by incorporating minimal supervision (less than $5$ labeled instances per intent). 
To summarize:

(i) We propose a novel, fully automated method, \mname{}, that jointly discovers newly emerging intents as well as domains in unlabeled user utterances.%, and hierarchically link related intents into domains. 

(ii) Unlike existing literature, \mname{} can generalize to diverse, open-world scenarios, and is independent of the intents and domains that it has been trained upon.

(iii) We extensively evaluate \mname{} on public benchmark datasets and real-world data from a commercial voice agent, and significantly outperform baselines across various empirical configurations. 




==> arXiv Discovering and Linking Novel User Intents from Text Utterances/methodology.tex <==
\section{Our Framework \mname{}}


Formally, we are given a corpus of training utterances $\mathcal{D_T}$ labeled with $S$ seen intents, and a corpus of unlabeled utterances $\mathcal{D_C}$ consisting of $U$ novel intents such that $S \cap U = \varnothing$. We propose a three-stage framework \mbox{\mname{}} that (i) classifies the incoming test utterance $x \in \mathcal{D_C}$ with one of the $S = (s_1, ..., s_S)$ seen intent labels or as an \textit{unseen} (\textit{novel}) intent; (ii) for utterances $\mathcal{D_X}$ predicted as having a novel intent, it discovers the latent intents $U = (u_1, ..., u_U)$ present in them; and (iii) links together mutually related novel intents discovered to form novel domains, and an intent-domain taxonomy. %We now describe these three stages of \mname{} below.


\subsection{Stage I: Detecting Instances with Novel Intents}
\label{sec:stage1}

We construct a two-step system to detect instances with \textit{novel} intents, inspired by the success of models pre-trained on large unlabeled corpora, like GPT~\cite{radford2018improving} and BERT~\cite{devlin2018bert}. 

\smallskip
\noindent \textbf{Step I:} 
Prior open classification literature has modeled the problem of finding \textit{novel} or \textit{unseen} classes as an $(S+1)$-class  classification problem, with $S$ \textit{seen} classes and an additional \textit{unseen} class. Labeled training data is available for the seen classes, and an input instance is classed as unseen if it does not belong to any of the seen classes~\cite{xu2019open,shu2018unseen,shu2017doc}. 
In a similar vein, to classify utterances as containing a novel intent or not, we learn a BERT based multi-class classifier (Figure~\ref{fig:stage1}). 
Given an input utterance $\bm{x}$, it is converted into a sequence of tokens to be input to BERT. A special classification embedding \texttt{[CLS]} is added as the first token. %, and another special token \texttt{[SEP]} is used for separating segments. The input representation is a concatenation of WordPiece embeddings~\cite{wu2016google}, positional embeddings, and the segment embedding. 
The output of BERT is an $n$-dimensional utterance encoding $(\bm{e_1},...,\bm{e_n})$. A multi-class intent classification layer on top of BERT predicts the utterance intent based on the final hidden state $\bm{e_1}$ of the \texttt{[CLS]} token as: 

\begin{center}
$y = \textrm{softmax}(\bm{W e_1} + \bm{b})$
\end{center}

\noindent where $\bm{W}$ is a task-specific parameter weight matrix. 
%Intuitively, the lower layer of the BERT model may contain more general information than the higher layers. 
We fine tune the parameters $\theta$ in different BERT layers with different learning rates as in~\cite{howard2018universal}, %. We split the parameters $\theta$ to be tuned into ${\theta_1, \theta_2, ..., \theta_L}$, where $\theta_l$ contains the parameters of the $l$-th layer of BERT. The parameters are then updated 
as follows:

\begin{center}
$\theta_t^l = \theta_{t-1}^l - \eta^l \nabla_{\theta_l} J(\theta)$
\end{center}

\noindent where $\eta_l$ and $\theta_l$ represent the learning rate and parameters respectively of the $l$-th BERT layer. $\nabla_{\theta_l} J(\theta)$ is the gradient with respect to the model's objective function. We set the base learning rate to $\eta^L$ and use $\eta^{l-1} = \xi.\eta^l$, where $\xi$ is a decay factor $\leq$ 1. %When $\xi < 1$, lower layers have a lower learning rate than higher layers. %When $\xi = 1$, all layers have the same learning rate, which is equivalent to the regular stochastic gradient descent (SGD). 
We fine-tune all BERT parameters as well as $\bm{W}$ jointly by maximizing the log-probability of the correct intent label.
%More details about these parameters are given in the Evaluation section.

%As part of training data for our multi-class classification model described above, we use the data consisting of utterances labeled with seen intents ($\mathcal{D_T}$). %However, unlike previous approaches, in order to classify an utterance $x$ as belonging to an unseen or novel intent, we utilize the following two sets of heuristics: 

For our $(S+1)$-class classification model described above, labeled training data $\mathcal{D_T}$ is available for the $S$ seen intents. We use \textit{out-of-domain} (OOD) intent detection datasets distinct from both $\mathcal{D_T}$ and $\mathcal{D_C}$, as training data for the $(S+1)$-th `novel' intent class. This OOD data comes from out-of-domain intent-labeled publicly available datasets (e.g. SNIPS~\cite{coucke2018}, ATIS~\cite{dahl1994}). Since we use already annotated, publicly available intent labeled data as OOD data, we don't require extra human annotation effort here. Note that while training, \mname{} only requires the information that the OOD intents do not overlap with those in $\mathcal{D_T}$ or $\mathcal{D_C}$, and \textit{not} the actual intent labels of the OOD data. 
However, if the OOD data is annotated with $m$ intent classes, \mname{} can use this information by fragmenting the $(S+1)^\text{th}$ class into $m$ classes, forming an $(S+m)$-class classification layer. Using $m$ classes may provide a better representation of the utterances likely to contain unseen intents (as shown in Section~\ref{sec:evalution}). An utterance classified into any of the $m$ classes is flagged as having a novel intent. 
% consisting of $m$ different intent classes. These OOD datasets can be any intent-labeled data that does not contain intents present in the $\mathcal{D_T}$ or $\mathcal{D_C}$ corpora. 
%If a test utterance is classified into any of the $m$ classes, we flag it as containing a novel intent. 

\smallskip
\textbf{Step II:} \mname{} employs an additional check as per the DOC algorithm~\cite{shu2017doc}. DOC learns statistical confidence thresholds for each seen intent class $s_i$. DOC thus captures instances that have been classified to one the $S$ seen intents with a low confidence. 
If the class-specific prediction probabilities for an input utterance are less than the thresholds learned for each seen intent $s_i$, that utterance is also classified as having a novel intent (see Figure~\ref{fig:stage1}). 


%\begin{itemize}

%\item We formulate our multi-class classification layer in Figure~\ref{fig:stage1} with $(S+m)$ intent class labels, for $S$ seen intents and $m$ possible novel or unseen intents. If a test utterance is classified into any of the $m$ classes, we flag it as containing a novel intent. As training data for the $m$ unseen intents, we use labeled data from \textit{out-of-domain} (OOD) datasets consisting of $m$ different intent classes. These OOD datasets can be any intent-labeled data that does not contain intents present in the $\mathcal{D_T}$ or $\mathcal{D_C}$ corpora. 

%\item We employ an additional check as per the DOC algorithm~\cite{shu2017doc} for those utterances that are classified as belonging to a seen intent with a confidence score below a learned threshold. DOC learns class-specific statistical confidence thresholds for each intent class. If the class-specific prediction probabilities for a test instance are less than their respective class thresholds, the instance is considered to contain a novel intent. 
%\end{itemize}


%A multi-class intent classification layer on top of BERT predicts the utterance intent. 

%\noindent The above approach categorizes all test utterances as containing either a seen or a novel intent.


\begin{figure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[height=4cm]{stage1}
  \caption{Detecting instances containing novel intents}
  \label{fig:stage1}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[height=4cm]{stage2}
  \caption{Discovering Novel Intent Categories}
  \label{fig:stage2}
\end{subfigure}
\caption{Overview of both stages of our approach, \mname{}}
\label{fig:advin}
\end{figure}



\subsection{Stage II: Discovering Novel Intent Categories}
\label{sec:stage2}

The output of the previous step of \mname{} gives us all utterances $\mathcal{D_X}$ that potentially contain a newly emerging intent. The next step is to discover the actual latent intent categories $U$ within $X$. We use complete-linkage, agglomerative hierarchical clustering~\cite{gowda1978agglomerative} to group together related utterances in $\mathcal{D_X}$, and find the potential novel intents $U$. %Starting with each utterance as a cluster, pairs of clusters are successively merged based on the distance between them. The merging stops when a certain maximum distance $\delta$ between clusters is reached. 

\smallskip

\noindent \textbf{Knowledge Transfer Component: }
Intuitively, humans seem to understand and categorize newly encountered objects based on the characteristics of similarities or differences that they learn from their prior knowledge of similar or comparable objects. We utilize a similar idea in order to learn the distance threshold $\delta$ for hierarchical clustering. That is, we transfer the knowledge learned from clustering the utterances containing seen intents $S$, to the utterances containing novel intents.
First, we perform hierarchical clustering on the labeled training data utterances $\mathcal{D_T}$, using the seen intents as ground truth cluster labels. %Starting with each utterance as a cluster, pairs of clusters are successively merged based on the distance between them. The merging stops when a certain maximum distance $\delta$ between clusters is reached. 
We obtain a distance value that maximizes the inter-intent distance between utterance clusters and minimizes the intra-intent distance within a cluster, by maximizing the F1 score of their clustering arrangement. 
In an ideal scenario, every obtained cluster $L_i$ represents a single seen intent. We also assume that utterances in the training set $\mathcal{D_T}$ of seen intents, as well as those in the unlabeled corpus $\mathcal{D_X}$ of newly emerging unseen intents come from similar distributions. %We can therefore transfer the distance threshold knowledge learned from clustering the seen intents to the novel or unseen intents. 
Our final step is then to \textit{transfer} this distance threshold $\delta$ learnt from the \textit{seen} intent utterances, to hierarchically cluster utterances in $\mathcal{D_X}$ containing novel or unseen intents. The distance threshold $\delta$ is defined as $\max\limits_{x \in L_i, x^p \in L_j} f(Emb(\bm{x}), Emb(\bm{x^p}))$ according to complete-linkage hierarchical clustering. Here, function $f(.)$ quantifies the distance between the embeddings $Emb(.)$ of an utterance pair $(\bm{x}$, $\bm{x^p})$ belonging to clusters $L_i$ and $L_j$ respectively.  %Hierarchical clustering stops when the distance $\delta$ between clusters is reached. 
%The value of $\delta$ for a clustering arrangement of the labeled training utterances $\mathcal{D_T}$ is the largest distance $dist(L_i, L_j)$ between every pair of clusters $L_i$ and $L_j$, and is given by: %$dist(C_i, C_j)$ is given by:

%\begin{center}
%$\delta = max_{i \neq j} dist(C_i, C_j)$
%\end{center}

%\noindent where $dist(C_i, C_j)$ is the distance between a pair of clusters $C_i$ and $C_j$, and is given by:


%\begin{center}
%\[
 %   dist(L_i, L_j) = \max\limits_{x \in L_i, x_p \in L_j} f(Emb(\bm{x}), Emb(\bm{x_p}))
%\]  

%\end{center}

%\noindent $f(Emb(\bm{x}), Emb(\bm{x_p}))$ denotes a distance function between the embeddings of a pair of utterances $\bm{x}$ and $\bm{x_p}$ (from Figure~\ref{fig:stage2}). These distances are given as input to the hierarchical clustering algorithm. 
We now describe how we learn the distance function $f$ between pairs of utterances.

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{Figures/stage2} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
\caption{Discovering Novel Intent Categories}
\label{fig:stage2}
\end{figure}
\end{comment}

\smallskip

\noindent \textbf{Learning Pairwise Utterance Distances for Clustering: }
We learn a neural network model to obtain utterance embeddings $Emb(.)$ for both the labeled corpus of seen intents ($\mathcal{D_T}$) and the unlabeled utterances detected to have novel intents ($\mathcal{D_X}$). %Figure~\ref{fig:stage2} displays the proposed architecture of our model. 
To train this model (see Figure~\ref{fig:stage2}), we create a training dataset from $\mathcal{D_T}$ comprising pairs of utterances $(x, x^p)$. Both $x$ and $x^p$ contain a seen intent. For each $x$, there are three possible choices for its paired utterance $x^p$: (i) $x^i$ containing the same domain and intent as $x$, (ii) $x^j$ containing the same domain but different intent than $x$, and (iii) $x^k$ containing a different domain and intent than $x$. Thus, $x^p \in \{x^i, x^j, x^k\}$. 
These utterance pairs $(x, x^p)$ are fed as input to an \texttt{EncoderNet}, which consists of a BERT transformer block. We use the same learning rate decay strategy of fine-tuning the BERT layers as earlier. Representations $E(\bm{x})$ and $E(\bm{x^p})$ are learned by the second last BERT layer (Figure~\ref{fig:stage2}).
The next layer on top of the \texttt{EncoderNet} blocks uses a distance function $d$ to compute pairwise representation distances, subject to the following bi-directional constraints: (i) the distance $d(E(x), E(x^i))$ between the representations of $x$ and $x^i$ should be less than $d(E(x), E(x^j))$; (ii) $d(E(x), E(x^i))$ between the representations of $x$ and $x^i$ should be less than $d(E(x), E(x^k))$; and (iii) the distance $d(E(x), E(x^j))$ between the representations of $x$ and $x^j$ should be less than the distance $d(E(x), E(x^k))$ between the representations of $x$ and $x^k$. These constraints utilize the semantic relationships between the utterance pairs containing different types of seen domains and seen intents. 
%Thus the next layer uses a distance function $d$ to compute the representation distances and enforce these constraints, which 
We then formulate a loss function $\mathfrak{L}$ to train our model, given by:

%\begin{center}
%$d(E(x), E(x^i)) + m_1 < d(E(x), %E(x^j))$
%$d(E(x), E(x^i)) + m_2 < d(E(x), %E(x^k))$
%$d(E(x), E(x^j)) + m_3 < d(E(x), %E(x^k))$
%\end{center}

\begin{align*}
%\mathfrak{L} &= \frac{1}{M} \sum\limits_{i, j, k} \{\max[0, m_1 + d(E(x), E(x^i)) - d(E(x), E(x^j)] \\ 
& \frac{1}{M} \sum\limits_{i, j, k} \{\max[0, m_1 + d(E(x), E(x^i)) - d(E(x), E(x^j)] + \alpha \max[0, m_2 + d(E(x), E(x^i)) - d(E(x), \\
& E(x^k)] + \beta \max[0, m_3 + d(E(x), E(x^j)) - d(E(x), E(x^k)] \}    
\end{align*}

\noindent where $m_1$, $m_2$, $m_3$ are predefined margins, $\alpha$ and $\beta$ are predefined weighting scalars and $M$ is the total number of utterance pairs $(x, x^p)$. We found such a loss formulation to outperform the popular contrastive loss~\cite{hadsell2006dimensionality} and triplet loss~\cite{schroff2015facenet} functions (Tables~\ref{tab:stage21} and~\ref{tab:stage22}). 
Next, a non-linear activation followed by a linear layer outputs embeddings $Emb(\bm{x})$ and $Emb(\bm{x^p})$ for the pair $(x, x^p)$. 
Finally, pairwise distances $f(Emb(\bm{x}), Emb(\bm{x_p}))$ are computed between all utterance pairs in this embedding space, to be given as input to %our Knowledge Transfer component performing 
hierarchical clustering. 
Note that we do not require any intent or domain labels for the unlabeled corpus $\mathcal{D_X}$ containing the unseen (novel) intents.
%We use euclidean distance in this work.  
%Once we have trained this model on the pairs of utterances containing seen intents, we learn embeddings and pairwise distances for the utterances in the test set $\mathcal{D_X}$, containing potentially novel or unseen intents. The pairwise distances learnt in the above manner for the labeled and unlabeled utterances are then given as input to the knowledge transfer component, that performs hierarchical clustering. 
 

%\smallskip

%\noindent \textbf{Linking Related Novel Intents into Novel Domains: }

%“We apply similar methodology as the knowledge transfer method. In order to prepare data for linking we perform the following steps (i) Assinging intent clusters to domain (ii) Obtain intent cluster representation (iii) Running the knowledge transfer method ..”


\subsection{Stage III: Linking Related Novel Intents into Novel Domains}
\label{sec:stage3}
After hierarchical clustering, \mname{} discovers a set of %groups or clusters of 
novel emerging intents. %, where utterances likely to contain the same novel intent are placed into the same cluster. 
We now aim to link together mutually related intents sharing the same broad functionality or the same semantic category into \textit{domains}. 
Hierarchical clustering already gives us a provision to `merge' together intents at the upper levels of the hierarchy based on distance. %This can be considered as related intents linking together. 
However, we find that using the domain labels available for the seen intents in a more direct manner leads to a better grouping of related novel intents into novel domains. We perform the following steps to link intents into domains, to create an intent-domain taxonomy:

(i) We assume that we have information regarding the domain of each seen intent in $S$. Assuming an ideal clustering in Section~\ref{sec:stage2}, each seen intent cluster $L_i$ will contain utterances belonging to a single seen intent $s_i \in S$. The domain label of cluster $L_i$ would be the domain of intent $s_i$ itself. However, $L_i$ may not be completely pure, i.e. it contains utterances with different seen intent labels. In such cases, we assign the domain label for $L_i$ as the domain of the intent of the majority of the utterances in $L_i$. 

(ii) We next obtain a representation $Emb_L(L_i)$ for each seen and novel intent cluster $L_i$, as the average of the embeddings $Emb(\bm{x})$ (from Figure~\ref{fig:stage2}) of all utterances $x \in L_i$. %We do this for both the seen and novel intent clusters.     

(iii) Finally, we re-use our Knowledge Transfer component to cluster the representations $Emb_L(L_i)$ of the seen intent clusters $L_i$ themselves. This time we use the seen \textit{domains} as ground truth cluster labels (instead of the seen \textit{intents} as in Section~\ref{sec:stage2}). As earlier, we obtain a distance threshold $\delta$ that maximizes the F1 score with respect to the seen domains. We then transfer this threshold to perform hierarchical clustering of the novel (unseen) intent clusters. 

\smallskip

\noindent Each cluster so obtained contains groups of related novel intents, representing novel domains. 
Thus, \mname{} creates a taxonomy of novel intents and domains from unlabeled user utterances.


%\subsection{Hyperparameters}




==> arXiv Discovering and Linking Novel User Intents from Text Utterances/relatedwork.tex <==
\section{Related Work} 
\label{sec:background}

%We describe two lines of research related to our work of discovering novel domains and intents from unlabeled text.

%\smallskip

%\noindent \textbf{Domain and Intent Detection:}
%Prior work on user intent detection encompasses two avenues: asynchronous, written communication (forums, blogs, tweets) and synchronous dialog from dialog agents such as Microsoft LUIS\footnote{https://www.luis.ai/}, Google Dialogflow\footnote{https://dialogflow.com/}, and Amazon Alexa\footnote{https://developer.amazon.com/alexa}. Supervised and semi-supervised learning models based on linguistic and sentiment features have been used to model racial intent on Tumblr~\cite{agarwal2017characterizing}, and purchase intent in social posts~\cite{gupta2014identifying,wang2015mining} and in discussion forums~\cite{chen2013identifying}. %Wang et al~\cite{wang2015mining} proposed a graph-based optimization approach for semi-supervised classification of tweets with a purchasing intent. Recent approaches have drawn upon progress in CNNs, RNNs, and transformer based language models to improve intent detection~\cite{xu2013convolutional,mesnil2015using,kim2016intent,liu2016attention,kim2017onenet,cai2017cnn,goo2018slot,xia2018,shivakumar2019spoken,castellucci2019multi} and domain detection~\cite{kim2018efficient,kim2018joint,zhang2018joint}. 
%Cai et al~\cite{cai2017cnn} used hierarchical clustering to learn a taxonomy of intent classes, and applied a hybrid CNN-LSTM model to classify the intent of medical queries. Performing slot filling jointly with intent detection has improved the performance of both tasks~\cite{kim2016intent,liu2016attention,zhang2016joint,wang2018bi}.  
Intent detection has been successfully performed in the literature via machine learning based approaches~\cite{tur2011sentence,jeong2008triangular,kim2016intent,ravuri2015comparative}, as well as deep learning models~\cite{sun2016weakly,xia2018,shivakumar2019spoken,castellucci2019multi,lin2019deep}. %\cite{ravuri2015comparative} performed a comparative study of different neural network architectures considering only lexical information of the utterance as features for intent detection. 
In recent years, intent detection has been jointly done with slot filling to improve its performance~\cite{xu2013convolutional,bhargava2013,liu2016attention,zhang2016joint,kim2017onenet,goo2018slot,wang2018bi}. However, the above approaches either require sufficient labeled data for each domain and intent, or some prior knowledge about the new intents to be discovered. \mname{} seeks to eliminate these restrictions.


%\smallskip

%\noindent \textbf{Open Classification:}
%Prior work classifies input instances into seen or unseen (during training) classes~\cite{scheirer2014probability,bendale2015towards,fei2016breaking,shu2017doc,xu2019open}. 
%Domain and intent detection 
Methods were proposed to recognize input texts belonging to novel domains~\cite{kim2018joint} and novel intents~\cite{lin2019deep,vedula2019towards}. However, unlike \mname{}, they do not jointly detect both novel domains and novel intents, cannot detect the number of novel domains and intents, and do not discover a taxonomy of the potential domain and intent types within user utterances. %likely to contain a novel domain or intent. 
Deep clustering networks~\cite{hsu2015neural} and Bayesian non-parametric models~\cite{dundar2012bayesian,akova2012self} were proposed to identify mixture components or clusters in data. But unlike \mname{}, the clusters identified cannot automatically be mapped to unique unseen categories. 
Our work %being completely unsupervised 
is also different from semi-supervised clustering techniques~\cite{fu2016semi,akova2012self,yi2015efficient,yi2013semi,hsu2015neural}, which lever small amounts of labeled data and require the classes to be discovered to be known beforehand. Having said that, we show the gains achieved by a semi-supervised version of \mname{}, in case prior knowledge is available about the novel intents (Table~\ref{tab:supervision}).
